The Geometry of Synchronization (Long Version)

We graft synchronization onto Girard's Geometry of Interaction in its most concrete form, namely token machines. This is realized by introducing proof-nets for SMLL, an extension of multiplicative linear logic with a specific construct modeling synchronization points, and of a multi-token abstract machine model for it. Interestingly, the correctness criterion ensures the absence of deadlocks along reduction and in the underlying machine, this way linking logical and operational properties.

==> local-macros.tex <==
% !TEX root = main.tex

%\newcommand{\ctxfour}{F}
\renewcommand{\ctxholep}[1]{\langle #1\rangle}
\newcommand{\ctxtwop}[1]{\ctxtwo\ctxholep{#1}}
\newcommand{\ctxthreep}[1]{\ctxthree\ctxholep{#1}}
\newcommand{\ctxfourp}[1]{\ctxfour\ctxholep{#1}}
\newcommand{\ctxfive}{G}
\newcommand{\ctxfivep}[1]{\ctxfive\ctxholep{#1}}
\newcommand{\ctxsix}{H}
\newcommand{\ctxsixp}[1]{\ctxsix\ctxholep{#1}}
\newcommand{\dom}[1]{dom(#1)}
\newcommand{\ctxenvf}[2]{#1(#2)}

%\newcommand{\sctxtwop}[1]{\sctxtwo\ctxholep{#1}}
\newcommand{\apctxp}[1]{\apctx\ctxholep{#1}}
\newcommand{\apctxtwop}[1]{\apctxtwo\ctxholep{#1}}
\newcommand{\apctxthreep}[1]{\apctxthree\ctxholep{#1}}

\newcommand{\nestto}[1]{\overset{#1}{\Rightarrow}}
\newcommand{\esmeas}[1]{|#1|_{[\cdot]}}

\newcommand{\unfsym}{\rotatebox[origin=c]{-90}{$\rightarrow$}}
\newcommand{\unf}[1]{#1\unfsym}
\newcommand{\relunf}[2]{\unf{#1}_{#2}}

\newcommand{\Opt}{Useful}
\newcommand{\opt}{useful}
\newcommand{\Nonopt}{Useless}
\newcommand{\nonopt}{useless}


%\newcommand{\toos}{\Rew{os}}

\newenvironment{varitemize}
{
\begin{list}{\labelitemi}
{
\setlength{\itemsep}{0pt}
 \setlength{\topsep}{0pt}
 \setlength{\parsep}{0pt}
 \setlength{\partopsep}{0pt}
 \setlength{\leftmargin}{15pt}
 \setlength{\rightmargin}{0pt}
 \setlength{\itemindent}{0pt}
 \setlength{\labelsep}{5pt}
 \setlength{\labelwidth}{10pt}}}
{
 \end{list}
}
\newcommand{\toos}{\Rew{os}}
\newcommand{\tonotdb}{\Rew{\neg\db}}

\newcommand{\deriv}{\rho}
\newcommand{\derivtwo}{\tau}
\newcommand{\derivthree}{\sigma}
\newcommand{\derivfour}{\pi}

\newcommand{\tobleft}{\Rew{l\beta}}

\newcommand{\sctximp}{\hat\sctx}

\newcommand{\tmsix}{q}
\newcommand{\tmp}{\tm'}
\newcommand{\tmtwop}{\tmtwo'}
\newcommand{\inst}{\lhd}
\newcommand{\lefttor}{\prec}

\newcommand{\redex}{R}
\newcommand{\redextwo}{S}
\newcommand{\sizedb}[1]{|#1|_{\db}}

% for references
\newcommand{\reflemma}[1]{Lemma~\ref{l:#1}}
\newcommand{\refth}[1]{Theorem~\ref{tm:#1}}
\newcommand{\refprop}[1]{Proposition~\ref{prop:#1}}
\newcommand{\refsect}[1]{Sect.~\ref{sect:#1}}
\newcommand{\reftab}[1]{Tab.~\ref{tab:#1}}
\newcommand{\refeq}[1]{(\ref{eq:#1})}
\newcommand{\refpoint}[1]{Point~\ref{p:#1}}
\newcommand{\refremark}[1]{Remark~\ref{rem:#1}}

\newcommand{\lefttortree}{\lefttor_{\Yup}}

\newcommand{\tmseven}{m}
\newcommand{\tmeight}{n}
\newcommand{\ls}{\lssym}
%\newcommand{\vsym}{{\tt v}}
%\newcommand{\tov}{\Rew{\vsym}}

\newcommand{\bctx}{B}
\newcommand{\bctxp}[1]{\bctx\ctxholep{#1}}
\newcommand{\bctxtwo}{B'}
\newcommand{\bctxtwop}[1]{\bctxtwo\ctxholep{#1}}


% call-by-value contexts
\newcommand{\cbvctx}{E}
\newcommand{\cbvctxtwo}{\cbvctx'}
\newcommand{\cbvctxthree}{\cbvctx''}
\newcommand{\cbvctxfour}{\cbvctx'''}
\newcommand{\cbvctxp}[1]{\cbvctx\ctxholep{#1}}
\newcommand{\cbvctxtwop}[1]{\cbvctxtwo\ctxholep{#1}}
\newcommand{\cbvctxthreep}[1]{\cbvctxthree\ctxholep{#1}}
\newcommand{\cbvctxfourp}[1]{\cbvctxfour\ctxholep{#1}}


